Greedy Bipartite Matching in Random Type Poisson Arrival Model

We introduce a new random input model for bipartite matching which we call the Random Type Poisson Arrival Model. Just like in the known i.i.d. model (introduced by Feldman et al. 2009), online nodes have types in our model. In contrast to the adversarial types studied in the known i.i.d. model, following the random graphs studied in Mastin and Jaillet 2016, in our model each type graph is generated randomly by including each offline node in the neighborhood of an online node with probability $c/n$ independently. In our model, nodes of the same type appear consecutively in the input and the number of times each type node appears is distributed according to the Poisson distribution with parameter 1. We analyze the performance of the simple greedy algorithm under this input model. The performance is controlled by the parameter $c$ and we are able to exactly characterize the competitive ratio for the regimes $c = o(1)$ and $c = \omega(1)$. We also provide a precise bound on the expected size of the matching in the remaining regime of constant $c$. We compare our results to the previous work of Mastin and Jaillet who analyzed the simple greedy algorithm in the $G_{n,n,p}$ model where each online node type occurs exactly once. We essentially show that the approach of Mastin and Jaillet can be extended to work for the Random Type Poisson Arrival Model, although several nontrivial technical challenges need to be overcome. Intuitively, one can view the Random Type Poisson Arrival Model as the $G_{n,n,p}$ model with less randomness; that is, instead of each online node having a new type, each online node has a chance of repeating the previous type.

==> known.tex <==
\chapter{Known Distribution Model}

\section{Edge-Weighted Matching}
%present simple 2-M algo and mention best current result (maryland paper)
In this section we consider the following stochastic problem: There is a bipartite graph $G(U,V,E)$ 
%where $A$
%corresponds to advertisers, $I$ corresponds to impressions and 
and a positive weight $w(e)$ associated with every edge $e \in E$. The graph $G$ is our \textit{type graph} with vertices in $U$ corresponding to the offline nodes and vertices in $V$ arriving online by being drawn with replacement from an I.I.D. distribution on $V$. For each $v \in V$ we are also given $r_{v}$, the number of times we expect that node to arrive. Let $n = \sum_{v\in V}r_{v}$ be the expected number of vertices arriving during the online phase. Let $D$ denote the distribution over $V$ defined by $Pr[v] = p_{v} = r_{v}/n$. The number $r_{v}$ is also called the \textit{arrival rate} of $v$. Throughout this chapter we are only concerned with instances having only integral arrival rates. As mentioned in \cite{HMZ}, wlog we can assume that $r_{v}=1, \forall v\in V$. This is true because a node $v$ with $r_{v}>1$ can be replaced by $r_{v}$ number of nodes identical to $v$, all having arrival rate 1. Note that when proving various approximation ratios we are assuming that $n\rightarrow +\infty$.\\

We are initially given access to $(G,D,n)$. In the online phase $n$ vertices are drawn i.i.d. from $V$. Upon the arrival of an online node $v$ we must either immediately assign it to a node $u\in U$ where $(u,v)\in E$, or not assign it at all. An offline node can be matched at most once. The objective is to maximize the total weight of the edges in the final matching.\\

More formally, let $D(v)$ be the set of draws of vertex type $v$ that arrive during the run of the algorithm. Let scenario $\hat{I} = \cup_{v\in V}D(v)$ be the set of vertices that arrive online. Let $\hat{G}(\hat{I})=(U,\hat{I},\hat{E})$ with $\hat{E}=\{(u,v'):(u,v)\in E, v' \in D(v)\}$ be the \textit{realization graph}. Given $(G,D,n)$ we want to find an algorithm $ALG$ such that $\mathbb{E}[ALG(\hat{I})]/\mathbb{E}[OPT(\hat{I})]\geq a$. In this case, we say that our algorithm achieves approximation ratio $a$ in expectation. As mentioned earlier, the expectation is both over $\hat{G}$ and any random choices made by the algorithm.\\
\begin{remark}
	The Display Ads problem can be reduced to this problem by repeating any offline node with capacity $c>1$, $c$ times.
\end{remark}



The way most algorithms for matching in this stochastic model work is by precomputing some matchings on the given type graph and then using them to guide the allocation during the online phase. What follows is a simple $1-1/e$ algorithm for our problem that uses a maximum weighted matching on the type graph.

\begin{algorithm}
	\caption{1-Suggested Matching}\label{1SM}
	\begin{algorithmic}[1]
		\State Compute a maximum weighted matching $M_{1}$ on the type graph $G$.
		\State When node $v$ arrives, if it is matched to a node $u\in U$ in $M_{1}$ and $u$ is so far unmatched, add $(u,v)$ to the final matching.
	\end{algorithmic}
\end{algorithm}

\begin{theorem}
	Algorithm 1-Suggested Matching has a competitive ratio of $1-1/e$\cite{HMZ}.
\end{theorem}

\begin{proof}
	To see why this is true, notice that the probability an edge from $M_{1}$ is included in the final matching is the probability that a node comes at least once. This probability is:
	$$\sum_{t=1}^{n} \frac{1}{n} (1-\frac{1}{n})^{t-1} \rightarrow 1-1/e$$
	This is the probability that at some time $t$, the corresponding online node arrives for the first time.
	Therefore we have that: $$\mathrm{E}[ALG] \geq w(M_{1})(1-1/e)$$
	Lastly, given that a maximum weighted matching on the type graph is an upper bound on the expected offline optimum solution (Manshadi et al.\cite{MGS}), the algorithm has a competitive ratio of $1-1/e$.
\end{proof}


%The algorithm uses the following matching LP formulation:
%\begin{align*}
%	\max \quad       & w^{T}p& & &\\
%	\text{s.t. \quad} & \sum_{v\in \delta(u)}p_{v} \leq 1,   & \forall u\in U & &\\
%	& \sum_{u\in \delta(v)}p_{v} \leq 1,   & \forall v\in V & &\\
%\end{align*}


To improve on the $1-1/e$ ratio, algorithms that use two (Haeupler at al. \cite{HMZ}) or more suggested matchings have been developed. Besides using more matchings, these algorithms use modified LPs to get offline solutions to the type graph in order to provide better upper bounds to the expected offline OPT, which is generally hard to compute exactly. The best current result for Edge-Weighted Matching in this model is achieved by an algorithm that uses three precomputed matchings and achieves a ratio of 0.705 (Brubach et al. \cite{Maryland}).





\subsection{Free Disposal}
Recall that under the \textit{free disposal} assumption, we are able to assign an arriving node to an already matched one, by displacing the matched edge (or one of the edges, if vertices have capacities) adjacent to that offline node. Seeing how without free disposal we can't get a competitive ratio better than $0$ in the adversarial model, this assumption seems to be quite powerful. In fact, the best results that don't make an assumption about large capacities, with the exception of algorithms in the \textit{known i.i.d. model}, always assume free disposal\footnote{It's worth noting that most of these results come from Submodular Welfare Maximization where the utility function that models edge-weighted matching naturally includes free disposal.}. It is interesting to note that no current algorithm for this stochastic model utilizes free disposal. Intuitively, it seems like the more information the online model provides, the less necessary this assumption becomes, yet it's still unclear to what extent it can be used to improve current bounds. The remainder of this chapter is an attempt at exploring the power of free disposal in the known i.i.d. model.\\\\
An important observation is the following:
\begin{remark}
	If every connected component of type graph $G$ has edges of equal weights, we cannot benefit from free disposal.\\
\end{remark}
The above is true for the simple reason that, given that we can't reassign nodes, we don't gain anything by replacing an assigned edge by another edge of equal weight. This means that for some type graphs, algorithms utilizing free disposal won't outperform algorithms that don't. In order to better understand the limits of the benefits of free disposal we will study an algorithm that adds this assumption on top of the common approach of using multiple precomputed matchings.\\
%Let $G(L\cup R, E)$ be the type graph. Assuming intergral arrival rates, a maximum weighted matching on the type %graph is an upper bound on the expected value of the offline optimum solution[further explanation + reference].
Let $M_{1}$ be a maximum weighted matching on the type graph $G$. Consider the modified graph $H$ that is constructed as follows: 
\begin{itemize}
	\item Remove edges that are in $M_{1}$.
	\item Remove any edge adjacent to an offline node that has been matched to an edge of bigger weight in $M_{1}$.
	\item For every edge in $H$ adjacent to a matched offline node in $M_{1}$, update its weight by subtracting the weight of the corresponding edge in $M_{1}$.
\end{itemize}
Let $M_{2}$ be a maximum weighted matching on $H$.\\
Now consider algorithm SFD (Stochastic Free Disposal) as shown below. Because of the construction of $H$, using a node from $M_{2}$ only adds weight to the final matching.
\begin{algorithm}
	\caption{SFD}\label{sfd}
	\begin{algorithmic}[1]
		\State When a node arrives for the first time, match it using $M_{1}$ if the corresponding offline node is available.
		\State When a node arrives for the second time, match it using $M_{2}$, possibly displacing an edge from $M_{1}$.
		\State If a node arrives three or more times, do nothing.
	\end{algorithmic}
\end{algorithm}

\begin{lemma}
	The expected weight of the matching produced by algorithm SFD is $(1-1/e)w(M1) + (1-2/e)w(M2)$.
\end{lemma}
\begin{proof}
	As mentioned earlier, the probability that an edge from $M_{1}$ is included in the final matching is the probability that a node comes at least once. This probability is: $$\sum_{t=1}^{n} \frac{1}{n} (1-\frac{1}{n})^{t-1} \rightarrow 1-1/e$$
	The probability that an edge from $M_{2}$ is included in the final matching is the probability that a node comes at least twice. Notice that because we updated the weights of $H$,  we can think of simply adding the weight of an edge from $M_{2}$, even though taking that edge might displace an edge from $M_{1}$. This simplifies the analysis. The probability of taking an edge from $M_{2}$ is the following:
	$$\sum_{t=1}^{n-1} (\frac{n-1}{n})^{t-1} \frac{1}{n} [1-(\frac{n-1}{n})^{n-t}] \rightarrow 1-2/e$$
	That is, the probability that a node arrives for the first time at time $t$ and then arrives at least once after that.
\end{proof}
The problem is that we can't make any assumption about the total weight of $M_{2}$ compared to the weight of $M_{1}$. The weight of $M_{2}$ is instance-specific and is in $[0,w(M_{1})]$, meaning that the competitive ratio of the algorithm SFD varies between $1-1/e\simeq 0.63$ and $2-3/e \simeq 0.89$. It is also worth pointing out that the above algorithm can be extended to utilize multiple matchings by making the same modification to $H$ and continuing until we get an empty graph. Notice also that picking an edge from the secondary matching  doesn't necessarily displace an edge.


\subsection{Experimental Results}
In this section we present some experimental results to evaluate this algorithm and get a better insight on free disposal as a heuristic in this model. Ideally we would use real advertising data to measure the algorithm's performance in this problem's most popular application, but such data is proprietary. Instead, we generated random type graphs and conducted the experiments by simulating the online phase. In the following tables, $n$ is the number of offline and online nodes of the type graph, $R$ constitutes the range in which the weights were uniformly chosen from, and $p$ is the probability there exists an edge between any two vertices. The values of the table show the average approximation ratio achieved by algorithm SFD against the (explicitly computed) optimum on the realization graph. In each case, a sample size of 1000 random type graphs was used.\\

\begin{center}
	\makebox[0pt]{\begin{tabular}{ c|c|c|c|c|c| } 
			$p=1/2$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
			\hline
			$n$ = 5& $0.795$ & $0.83$ &$0.846$  &$0.854$ &$0.884$\\
			\hline
			$n$ = 10&$0.675$ & $0.734$ & $0.776$  &$0.788$ & $0.789$\\
			\hline
			$n$ = 50&$0.637$ & $0.633$ & $0.657$  &$0.689$ & $0.697$\\
			\hline
			$n$ = 100&$0.635$ & $0.631$ & $0.628$ & $0.672$ & $0.677$\\ 
			\hline
			%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
			%\hline
	\end{tabular}}
\end{center}
\hfill \\\\
\begin{center}
	\makebox[0pt]{\begin{tabular}{ c|c|c|c|c|c| } 
			$p=1/5$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
			\hline
			$n$ = 5& $0.835$ & $0.85$ &$0.861$  &$0.875$ &$0.869$\\
			\hline
			$n$ = 10&$0.792$ & $0.817$ & $0.846$  &$0.85$ & $0.854$\\
			\hline
			$n$ = 50&$0.61$ & $0.624$ & $0705.$  &$0.725$ & $0.725$\\
			\hline
			$n$ = 100&$0.607$ & $0.601$ & $0.65$ & $0.686$ & $0.688$\\ 
			\hline
			%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
			%\hline
	\end{tabular}}
\end{center}
\hfill \\\\
\begin{center}
	\makebox[0pt]{\begin{tabular}{ c|c|c|c|c|c| } 
			$p=1/10$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
			\hline
			$n$ = 5& $0.719$ & $0.733$ &$0.714$  &$0.743$ &$0.735$\\
			\hline
			$n$ = 10&$0.846$ & $0.87$ & $0.867$  &$0.862$ & $0.881$\\
			\hline
			$n$ = 50&$0.628$ & $0.698$ & $0.761$  &$0.777$ & $0.774$\\
			\hline
			$n$ = 100&$0.597$ & $0.616$ & $0.7$ & $0.72$ & $0.723$\\
			\hline
			%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
			%\hline
	\end{tabular}}
\end{center}
\hfill \\\\
\hfill \\\\
In some settings the competitive ratio achieved by SFD seems to improve on the most recent 0.705 result \cite{Maryland}, but in others it's barely better than $1-1/e$ or even slightly worse. Because of how much the results vary based on the weight range and the probability of edge existence, the performance of this algorithm depends on the application it's used for and the setting that most accurately models the corresponding data. This is just one way that free disposal can be utilized in this model and there are various other approaches worth exploring. Online matching algorithms fall into two categories, \textit{adaptive} and \textit{non-adaptive}. When a new node arrives, an adaptive algorithm is allowed to consider the vertices arrived thus far and previous assignments before deciding whether to match the new node or discard it. A non-adaptive algorithm specifies all of its actions before the beginning of the online phase. Because of the information provided in the known distribution model, most work has been focused on non-adaptive algorithms using precomputed matchings in ways as described earlier. There is still an open question about how much better we can do using adaptive algorithms and whether adaptiveness allows for better utilization of free disposal is a possibility worth investigating.

\chapter{Random Type-Graph Model}

The variables used in the experiments of algorithm SFD implicitly define a stochastic model that is different compared to the known distribution model. In this chapter we formalize this stochastic model that we think is an interesting one and is worth using to analyze algorithms. Lastly we provide some additional experimental data to see how the Greedy matching algorithm performs in this model.

\section{Model Description}
%$G_{n,n,p,R}$
First, some notation on random graphs:
\begin{definition}
	$\mathcal{G}_{n,n,p}$ is the random bipartite graph with each of the two node sets having size $n$ and where the existence of each of the $n^{2}$ possible edges is decided independently with probability $p$.\\
\end{definition}

\begin{definition}
	$\mathcal{G}_{n,n,p,R}$ is the graph $\mathcal{G}_{n,n,p}$ with each edge having a uniformly random weight in $[1,R]$.\\
\end{definition}

In the \textit{random type-graph model} (\textbf{RTG}), we are given access to a $\mathcal{G}_{n,n,p,R}$ type graph and the node arrival process is the same as in the known i.i.d. model. The motivation behind this model is proving competitive ratios for various value combinations of $n$, $p$, and $R$. This would allow us to model application-specific settings and get a more relevant performance guarantee. Furthermore, since the competitive ratio of an algorithm in the know i.i.d. model holds for any type graph, it will also hold for a random one. Therefore, the following is true:
$$C.R.(\text{\textit{Known IID}})\leq C.R.(RTG)$$


\section{Perfect Matchings}
In this section we present a theorem about perfect matchings that gives some insight on the performance of algorithm SFD. Let $\mathcal{G}_{n,n,p}$ be the random graph as defined earlier and $\delta(\mathcal{G}_{n,n,p})$ be the minimum degree of graph $\mathcal{G}_{n,n,p}$. The following theorem was proved by Erd\H{o}s and R\'enyi \cite{ErdosRenPM}.
\hfill \\\\
\begin{theorem}
	Let $\omega = \omega(n)$, $c>0$ be a constant, and $p=\frac{logn+\omega}{n}$. Then:
\begin{center}
	$	  \lim_{n\rightarrow \infty}\Pr(\mathcal{G}_{n,n,p})\text{ has a perfect matching})= \begin{cases} 0 &\mbox{if } \omega \rightarrow -\infty \\ 
	e^{-2e^{-c}} & \mbox{if } \omega \rightarrow c \\
	1 &\mbox{if } \omega \rightarrow \infty \end{cases}$
\end{center}
Moreover,
$$\lim_{n\rightarrow \infty}\Pr(\mathcal{G}_{n,n,p})\text{ has a perfect matching})=\lim_{n\rightarrow  \infty}\Pr(\delta(\mathcal{G}_{n,n,p})\geq 1)$$\\
\end{theorem}

Recall that a perfect matching includes all the vertices of the graph.
To see how this theorem on unweighted graphs is relevant to our algorithm, consider the subgraph of $\mathcal{G}_{n,n,p,R}$ that only contains edges of weight $R$. If this subgraph has a perfect matching, $M_{1}$ will find it and $M_{2}$ will be empty, leaving no allocation rule for a node that comes more than once and the algorithm achieving a competitive ratio of $1-1/e$. Another way to describe this subgraph is by the random graph $\mathcal{G}_{n,n,p/R}$. Therefore we have that:
$$\Pr(M_{2} = \emptyset) \geq \Pr(\mathcal{G}_{n,n,p/R} \text{ has a perfect matching})$$ and 
$$\Pr(\mathcal{G}_{n,n,p/R} \text{ has a perfect matching}) \rightarrow 1 \text{,  as  }\frac{p}{R} \rightarrow +\infty$$\\
This observation provides some additional insight into the limits of algorithm SFD and any non-adaptive algorithm that uses a maximum weighted matching on the type graph as a primary allocation rule.


\section{Greedy}
Greedy algorithms is often the first algorithmic paradigm explored when considering many problems and matching is no exception. For the edge-weighted case, the conventional greedy algorithm (referred to as \textbf{Greedy}) assigns the arriving node to the available neighbor with the maximum weight. This algorithm currently achieves the best known competitive ratios of $1-1/e$ and $0.51$ for the unknown i.i.d. and random order models respectively. In the adversarial model it achieves a ratio of $1/2$ which was only recently broken by a more sophisticated randomized algorithm that achieves a slightly better competitive ratio of $0.5018$ (\cite{mortezaADV}). This was an important result as it was the first evidence that edge-weighted matching is strictly easier than submodular welfare maximization for which the optimal competitive ratio in the adversarial model is $1/2$. In the known i.i.d case, the only known lower bound on the competitive ratio of Greedy is $1-1/e$ and that follows from the unknown i.i.d. model\footnote{This competitive ratio for Greedy was shown for the more general problem of submodular welfare maximization.}. In this section we present some experimental data on the performance of Greedy in the RTG model, which is getting very good results and outperforming algorithm SFD. We also include data on the greedy algorithm that uses free disposal. This algorithm assigns the newly arrived vertex to the offline node that maximizes its \textit{marginal gain}, which is defined as the result of subtracting the weight of the edge currently matched to the corresponding offline node from the weight of the edge of the online node that just arrived. The tables below follow the same format as in the previous chapter.\\\\

%-----------------------------------------------------------------\\

%\begin{center}
	\begin{table}
	\makebox[450pt]{
		\begin{tabular}{ c|c|c|c|c|c| } 
			$p=1/2$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
			\hline
			$n$ = 5& $0.939$ & $0.934$ &$0.924$  &$0.924$ &$0.916$\\
			\hline
			$n$ = 10&$0.914$ & $0.91$ & $0.906$  &$0.905$ & $0.901$\\
			\hline
			$n$ = 50&$0.982$ & $0.959$ & $0.929$  &$0.929$ & $0.928$\\
			\hline
			$n$ = 100&$0.991$ & $0.98$ & $0.95$ & $0.95$ & $0.95$\\ 
			\hline
			%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
			%\hline
%			\caption*{Greedy}
	\end{tabular}

\quad
\begin{tabular}{ c|c|c|c|c|c| } 
	$p=1/2$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
	\hline
	$n$ = 5& $0.935$ & $0.955$ &$0.966$  &$0.975$ &$0.968$\\
	\hline
	$n$ = 10&$0.916$ & $0.924$ & $0.939$  &$0.94$ & $0.941$\\
	\hline
	$n$ = 50&$0.981$ & $0.962$ & $0.936$  &$0.936$ & $0.936$\\
	\hline
	$n$ = 100&$0.991$ & $0.981$ & $0.954$ & $0.954$ & $0.954$\\ 
	\hline
	%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
	%\hline
\end{tabular}

}
\caption*{Greedy \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad Greedy + FD}
\end{table}
%\end{center}



%\begin{center}
	\begin{table}

	\makebox[450pt]{
		\begin{tabular}{ c|c|c|c|c|c| } 
			$p=1/5$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
			\hline
			$n$ = 5& $0.94$ & $0.944$ &$0.925$  &$0.93$ &$0.92$\\
			\hline
			$n$ = 10&$0.939$ & $0.936$ & $0.923$  &$0.919$ & $0.91$\\
			\hline
			$n$ = 50&$0.931$ & $0.891$ & $0.898$  &$0.894$ & $0.894$\\
			\hline
			$n$ = 100&$0.968$ & $0.935$ & $0.912$ & $0.913$ & $0.913$\\ 
			\hline
			%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
			%\hline
	\end{tabular}
\quad
\begin{tabular}{ c|c|c|c|c|c| } 
	$p=1/5$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
	\hline
	$n$ = 5& $0.941$ & $0.957$ &$0.957$  &$0.963$ &$0.956$\\
	\hline
	$n$ = 10&$0.948$ & $0.963$ & $0.973$  &$0.976$ & $0.974$\\
	\hline
	$n$ = 50&$0.931$ & $0.901$ & $0.92$  &$0.922$ & $0.922$\\
	\hline
	$n$ = 100&$0.968$ & $0.942$ & $0.925$ & $0.926$ & $0.925$\\ 
	\hline
	%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
	%\hline
\end{tabular}
}
\caption*{Greedy \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad Greedy + FD}
\end{table}
%\end{center}


%\begin{center}
	\begin{table}[htb]
	\makebox[450pt]{\begin{tabular}{ c|c|c|c|c|c| } 
			$p=1/10$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
			\hline
			$n$ = 5& $0.799$ & $0.799$ &$0.784$  &$0.796$ &$0.79$\\
			\hline
			$n$ = 10&$0.978$ & $0.96$ & $0.941$  &$0.942$ & $0.943$\\
			\hline
			$n$ = 50&$0.879$ & $0.892$ & $0.893$  &$0.891$ & $0.892$\\
			\hline
			$n$ = 100&$0.924$ & $0.886$ & $0.892$ & $0.892$ & $0.891$\\ 
			\hline
			%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
			%\hline
	\end{tabular}
\quad
\begin{tabular}{ c|c|c|c|c|c| } 
	$p=1/10$& $R$ = 1 & $R$ = 2 & $R$ = 10 & $R$ = 100 & $R$ = 1000\\
	\hline
	$n$ = 5& $0.813$ & $0.811$ &$0.818$  &$0.81$ &$0.8$\\
	\hline
	$n$ = 10&$0.977$ & $0.986$ & $0.987$  &$0.99$ & $0.989$\\
	\hline
	$n$ = 50&$0.883$ & $0.915$ & $0.938$  &$0.94$ & $0.94$\\
	\hline
	$n$ = 100&$0.924$ & $0.897$ & $0.919$ & $0.921$ & $0.921$\\ 
	\hline
	%$n$ = 1000&$-$ & $-$ & $-$  & $-$ & $-$\\ 
	%\hline
\end{tabular}
}
\caption*{Greedy \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad  \quad \quad Greedy + FD}
\end{table}
%\end{center}
\hfill \\\\

These results show that Greedy performs much better in the distribution models than the lower bound of $1-1/e$ seems to indicate. In fact, these ratios are much better even compared to the more sophisticated algorithms for the known i.i.d. model for which a much better lower bound on the competitive ratio is known. This seems to indicate that for the greedy algorithm, random instances of this matching problem are much easier than worst case instances. As expected, Greedy with free disposal only does better than the conventional greedy algorithm, except for the case of $R=1$ where displacing an edge is pointless.
To try and explain why Greedy works so well in the RTG model, we reference a theorem about the performance of Greedy on the unweighted graph $\mathcal{G}_{n,n,p}$ that is constructed in an online fashion. The following theorems and corollary come from the work of Jaillet and Mastin \cite{MastJailGnnp}.

\begin{theorem}
	Let $\mu_{G}(n,n,c/n)$ denote the matching size obtained by the greedy algorithm on the graph
	$\mathcal{G}_{n,n,p}$, where $p = c/n$ and $c > 0$ is a constant. Then asymptotically almost surely:
	$$\frac{\mu_{G}(n,n,c/n)}{n} = 1-\frac{log(2-e^{-c})}{c}+o(1)$$
\end{theorem}
\begin{theorem}
	The performance ratio $R_{G}(p(n))$ of Greedy on $\mathcal{G}_{n, n, p}$, for all valid functions $p =
	p(n)$, satisfies:
	\begin{align*}
	R_{G}(p(n)) & = 1 &p(n) = o(1/n)\\
	R_{G}(p(n)) &\geq \frac{c-log(2-e^{-c})}{2c-(\gamma^{*} +\gamma_{*} + \gamma^{*}\gamma_{*})} &p(n)=c/n \\
	R_{G}(p(n)) & = 1 &p(n) = \omega(1/n)\\
	\end{align*}
\end{theorem}
\begin{corollary}
	The performance ratio of Greedy on $\mathcal{G}_{n, n, p}$ for all valid functions $p = p(n)$ satisfies:
	$$R_{G}(p(n))\geq 0.837$$\\
\end{corollary}

Based on the experimental data provided and the fact that Greedy performs really well on random graphs indicate that a similar result like the one above might hold in the RTG model both for the unweighted and weighted cases.
 

\section{Poisson Arrivals}
A model similar to RTG is the \textit{Poisson arrivals model}. We are given a type graph $\mathcal{G}_{n,n,p}$ that specifies the neighborhood of each type. Let $Y_{i}$ be the random variable representing the number of times type $i$ arrives. In the Poisson arrivals model, we have that $Y_{i}\sim \text{ Poisson(1)}$.
We argue that this is a natural model to study for the following reasons. In the conventional known i.i.d. model, we have that $Y_{i}\sim \text{ Bin($n,\frac{1}{n}$)}$ and it holds that Bin($n,\frac{1}{n}$)$\xrightarrow{\mathcal{D}}$ Poisson($1$), while most proofs of competitive ratios already make the assumption that $n\rightarrow +\infty$. Additionally, we remove  the dependency $Y_{1}+\dots+Y_{n}=n$ that exists in the conventional model and we allow for the total number of online nodes to be greater or less than $n$.\\\\%[Poisson also used to model arrivals in other real scenarios]
A way of thinking about the arriving nodes is the following: A number of nodes of each type is generated following the Poisson distribution. These nodes are then randomly permuted and are presented to the algorithm in an online fashion. The idea for studying algorithms under the Poisson arrivals model comes from the generalization of some results in a similar model by Jaillet and Lu (\cite{stochasticFlowPois}). Motivated by the performance of Greedy on the graph $\mathcal{G}_{n,n,p}$, we prove the two following theorems.\\
\begin{theorem}
	On type graph $\mathcal{G}_{n,n,p}$ with Poisson arrivals and $p(n)=o(1/n)$, the performance of Greedy satisfies $C.R.(Greedy) = 1$.
\end{theorem}
\begin{proof}{(similar to proof of Lemma 2 in \cite{MastJailGnnp})}
	Let $M$ be the matching produced by Greedy and $M^{*}$ be a maximum matching on the realization graph. Let $N(v)$ be the set of neighbors of node $v$. We consider the number of isolated edges in the type graph. An edge $(i,j)$ is isolated if $N(i)=\{j\}$ and $N(j)=\{i\}$. The probability of an isolated edge between $i$ and $j$ is:
	$$\Pr((i,j) \text{ is isolated edge })=p(1-p)^{2n-2}$$
	Every isolated edge will be matched by algorithm Greedy, therefore:
	$$\mathbb{E}[|M|]\geq n^{2} (1-\frac{1}{e})p(1-p)^{2n-2}$$
	The size of a maximum matching $|M^{*}|$ is upper bounded in expectation by the expected number of edges $n^{2}(1-\frac{1}{e})p$, therefore:
	$$\frac{\mathbb{E}[|M|]}{\mathbb{E}[|M^{*}|]}\geq (1-p)^{2n-2}=(e^{-o(\frac{1}{n})})^{2n-2}=e^{-o(1)}\rightarrow 1$$
\end{proof}
\begin{theorem}
	On type graph $\mathcal{G}_{n,n,p}$ with Poisson arrivals and $p(n)=\omega(1/n)$, the performance of Greedy satisfies $C.R.(Greedy) = 1$.
\end{theorem}
\begin{proof}
	Let $p(n)=\frac{g(n)}{n}$ and $k=\frac{n}{\sqrt{g(n)}}$. Since $p(n)=\omega(1/n)$, we have that $\frac{1}{\sqrt{g(n)}}=o(1)$.
	\hfill \\\\
	For the analysis, we will think of the online process in the following way. We pick a type $i$, generate $Y_{i}$ nodes of this type, and present them to the algorithm for matching. Again, we have that $Y_{i}\sim$ Poisson($1$). When nodes of a type are generated, assume there are at least $k$ offline nodes unmatched and let $X\sim$ Bin($k,p$) be the number of neighbors of type $i$ among those offline nodes. More specifically, we assume that the algorithm matches less than $n-k$ offline nodes in total, so $k$ nodes are always available. In the case where more than $n-k$ nodes are matched, since $k=o(n)$, we get a trivial competitive ratio of $1-o(1)$.
	\hfill \\\\
	Assuming there are at least $k$ available nodes, we will prove that $\Pr(X\geq Y_{i}) \geq 1-o(1)$. For variable $Y_{i}$ we have the following:
	\begin{align*}
		&P(Y_{i} = m)=\frac{1}{m!} \cdot \frac{1}{e} \\
		&P(Y_{i} \geq m)\leq \frac{1}{e}\sum_{j=m}^{+\infty}\frac{1}{j!} \leq \frac{1}{m!}\leq \frac{1}{2^{m}}  \\
		 &P(Y_{i} \geq g(n)^{1/100}) \leq \frac{1}{2^{g(n)^{1/100}}}  \quad (1)\\
	\end{align*}
	For variable $X$ we have the following:
	$$Var(X) = k\cdot p(1-p)\approx \sqrt{g(n)}$$
	$$\mu = k\cdot p = \sqrt{g(n)}$$
	Chebyshev's inequality:
	$$\Pr(|X-\mu|\geq c)\leq \frac{Var(x)}{c^{2}}=\frac{\sqrt{g(n)}}{c^{2}}$$
	$$\Pr(|X-\mu|\geq g(n)^{1/3})\leq \frac{\sqrt{g(n)}}{g(n)^{2/3}}=\frac{1}{g(n)^{1/6}}\quad (2)$$
	From $(1)$ and $(2)$ we have that:\\
	$$\Pr(X\geq Y_{i})\geq \Pr(Y_{i}\leq g(n)^{1/100}  \wedge  X\geq \sqrt{g(n)}-g(n)^{1/3} )
	\geq 1-\frac{1}{g(n)^{1/6}}-\frac{1}{2^{g(n)^{1/100}}}\rightarrow1$$\\
%	---------------------------\\
	From the above, and because of the principle of delayed decisions, we get the following:\\
	$$\mathbb{E}[\text{\# of times type i is matched}]\geq \mathbb{E}[\text{\# of times type i is generated}]\cdot\Pr(X\geq Y_{i})\geq \mathbb{E}[Y_{i}]\cdot(1-o(1))$$\\
	and since $\mathbb{E}[OPT]\leq \mathbb{E}[Y_{i}]$, we get that:
	$$C.R.(Greedy)\rightarrow 1$$
\end{proof}
\hfill \\\\
The intermediate case of $p(n)=c/n$ is still open.



==> minimizer.tex <==
\begin{lemma}
\label{lem:minimizer}
Let $p_1, \ldots, p_n$ be parameters and fix $k \in \mathbb{Z}_{\ge 0}$ and $\tau \in \mathbb{R}_{\ge 0}$. Define
\[ R(p_1, \ldots, p_n) = \mathbb{E}(\min(\Ber(p_1) + \cdots + \Ber(p_n),k)).\]
Then the minimum of $R$ subject to $\sum_i p_i = \tau$ is achieved at $p_1 = \cdots = p_n = \tau/n$.
\end{lemma}
\begin{proof}
Suppose that $p = (p_1, \ldots, p_n)$ are such that $\sum_i p_i = \tau$ and that $p_1 \neq p_2$. We will show that $q=((p_1 + p_2)/2, (p_1 + p_2)/2, p_3, \ldots, p_n)$ results in a smaller value of $R$, i.e., that $R(q) \le R(p)$. Of course, there is nothing special about $p_1$ and $p_2$, and the same argument holds for all pairs $p_i$ and $p_j$ with $i \neq j$. Thus, by repeatedly averaging pairs of coordinates we can decrease the value of the objective, in the limit getting the minimizing values $p_1 = p_2 = \ldots = p_i = \tau/n$.

Let $p' = (p_2, p_1, p_3, \ldots, p_n)$. Clearly, we have $R(p) = R(p')$. It suffices to show that $R$ is convex on the interval $[p, p'] = \{ \alpha p + (1-\alpha) p' \mid \alpha \in [0,1]\}$. If $R$ is convex on the interval, we get $R(q) = R((p+p')/2) \le R(p)/2 + R(p')/2 = R(p)$.

Fix values of $p_3, \ldots, p_n$ and consider the following function:
\begin{align*}
     f(x, y) &= x y \mathbb{E}\left( \min\left( 2+ \sum_{i \ge 3}\Ber(p_i), k\right) \right)\\
&+ ((1-x) y + (1-y) x) \mathbb{E}\left(\min\left( 1+ \sum_{i\ge 3} \Ber(p_i), k\right) \right)\\
&+(1-x)(1-y) \mathbb{E}\left( \min\left( \sum_{i \ge 3}\Ber(p_i), k\right) \right)\\
&= x y a_1 + ((1-x) y + (1-y)x)a_2 + (1-x)(1-y)a_3,
\end{align*}
where the coefficients $a_i$ are defined to be the values of the respective expectations. Note that we have $f(p_1, p_2) = R(p_1, p_2, \ldots, p_n)$. Convexity of $R$ on the interval $[p,p']$ is equivalent to convexity of $f$ in the direction $v=(p_2-p_1, p_1-p_2)$.

The Hessian of $f$ is 
\[
H = 
\begin{bmatrix}
0 & a_1 - 2a_2 + a_3 \\
a_1 - 2a_2 + a_3 & 0
\end{bmatrix}
\]
The sign of the bilinear form associated with $H$ and evaluated in the direction of interest tells us whether the function is convex or concave in that direction. We are interested in the direction $v = (p_2 - p_1, p_1 - p_2)$. Evaluating $v^T H v = -2 (a_1 - 2a_2 + a_3)(p_1-p_2)^2$. To finish the proof it suffices to prove that $a_1 - 2 a_2 + a_3 \le 0$, because then $v^T H v \ge 0$ and $f$ is convex in the direction $v$. Thus we need to determine the sign of the following expression:
\[
\mathbb{E}\left( \min( 2+W, k) - 2 \min(1+W, k) + \min(W, k) \right),
\]
where $W = \sum_{i \ge 3} \Ber(p_i)$. Consider three cases:
\begin{description}
\item[Case 1:] $W \ge k$ --- the expression inside the expectation becomes $k-2k+k=0$.
\item[Case 2:] $W = k-1$ --- the expression inside the expectation becomes $k-2k+(k-1)=-1$.
\item[Case 3:] $W \le k-2$ --- the expression inside the expectation becomes $W+2-2(W+1)+W=0$.
\end{description}
This shows that $a_1 - 2a_2-a_3 \le 0$ finishing the proof of the lemma.
\end{proof}
